Measurements of the Most Significant Software Security Weaknesses

In this work, we provide a metric to calculate the most significant software security weaknesses as defined by an aggregate metric of the frequency, exploitability, and impact of related vulnerabilities. The Common Weakness Enumeration (CWE) is a well-known and used list of software security weaknesses. The CWE community publishes such an aggregate metric to calculate the `Most Dangerous Software Errors'. However, we find that the published equation highly biases frequency and almost ignores exploitability and impact in generating top lists of varying sizes. This is due to the differences in the distributions of the component metric values. To mitigate this, we linearize the frequency distribution using a double log function. We then propose a variety of other improvements, provide top lists of the most significant CWEs for 2019, provide an analysis of the identified software security weaknesses, and compare them against previously published top lists.

==> Archive/AssaneSection.tex <==
%%% General security metrics
Modern’s society constant need to improve computer and information security has motivated a widespread interest in deriving metrics for security. Indeed, as stated by Lord Kelvin, \emph{you cannot improve if you cannot measure}. Decision-makers need information about the utility of different security options to make appropriate decisions and to determine how well an organization is meeting its security objectives. Software vendors must provide (to end-users) quantifiable proof that their proposed solutions are achieving the desired security level. End-users must be able to verify such claim. They also need a measuring stick to assess risk related to using a given solution, as risk management requires that one solution be evaluated against an alternate one. This has led to many efforts devoted to deriving qualitative ways \cite{guide_secu} as well as quantitative ways \cite{ ou2011quantitative} to measure security. The present paper sits within the latter group.

% Critics of security metrics
Providing useful metrics for software security has been identiﬁed as a diﬃcult undertaking mainly because of the lack of a ground truth to assess security metrics. This has prompted members of the software security community to doubt about our ability to succeed in our attempts to quantify security. Bellovin was among the first \cite{Bellovin2006} to argue about the infeasibility of software security metrics. \cite{Cox-limit2008} discusses the limitations of the celebrated ``Risk = Threat × Vulnerability × Consequence'' model that is widely used. In \cite{Verendel2009QuantifiedSI} Verendel presents a critical survey of results and assumptions made in the community to quantify security. After reviewing over 100 articles, he concludes that the validity of most methods is still strikingly unclear. Many reasons explain this invalidity:  lack of validation, lack of comparison against empirical data, and the fact that many assumptions in formal treatments are not empirically well-supported in operational security.

Although we agree that the field of security metrics is a difficult area of scientific research, we believe that acceptable solutions must be found in order to make security decisions and to evaluate whether or not a security posture has improved or declined. The CWE \cite{CWE} is widely agreed to be one of such acceptable solutions. This paper considers the CWE, identifies some of its weaknesses, and proposes  a way to improve it.

%surveys
Despite the doubts raised by some authors,  there has been substantial efforts to produce security metrics. \cite{Verendel2009QuantifiedSI} surveys the literature of security metrics published between 1981 and 2008. More efforts can be found in \cite{Purboyo2011}, \cite{Pendleton2017}, and \cite{MorissonSMS}. This latter survey considers how to measure system-level security by proposing a security metrics framework based on vulnerabilities, defense power, attack or threat severity, and situations (state of system). The authors discuss the state-of-art of existing security metrics and their advantages and disadvantages. They also discuss open research questions in the security metrics research domain and suggest key factors to improve security.

% Discovery tools/methods/DB (Weakness, vulnerability, exploit, attack)
% Prioritizing TOP-X
% Mitigating

Improving software security requires the collaboration of several actors, including: language designers, compiler writers, educators, assurance tool developers, researchers, vulnerability trackers, and software engineers. Such a collaboration cannot succeed if these actors do not ``speak the same language’’. This is what motivated the development and the adoption of widely agreed taxonomies for weaknesses \cite{CWE}, vulnerabilities \cite{CVE}, as well as attacks \cite{CAPEC}. Once broadly accepted definitions and classifications are developed, the key elements pertaining to security can be collected and stored in databases for the needed future analysis. Several such databases have been implemented and are publicly available. They include the  CWE list \cite{NVDCWE}, the CVE list \cite{CVE}, the NVD \cite{NVD}, the exploit DB \cite{ExploitDB}, and the Common Attack Pattern Enumeration and Classification   \cite{CAPEC}. This work is particularly focused on the CWE. It also leverages the CVE and the NVD.

These databases contain sometimes up to thousands of items. From an operational point of view and because of the limited available resources  (manpower, time, money, etc.), one needs to focus on the most ``important’’ items (weakness, vulnerability, exploit, or attack). But finding the most important items requires a metric to compare them.  This has sparked a widespread interest in deriving metrics for security. A number of them can be found in the survey papers \cite{Verendel2009QuantifiedSI}, \cite{Purboyo2011}, \cite{Pendleton2017}, and \cite{MorissonSMS}. The CWE project has also introduced the Common Weaknesses Scoring System (CWSS) \cite{CWSS} and the Common Weakness Risk Analysis Framework (CWRAF) \cite{CWRAF}, which are used in conjunction to provide to an organization with a tailored  list of most important weaknesses. 

Using these metrics, we can generate ``Top XX’’ lists such as the MITRE CWE Top25 \cite{MitreTop25} and the OWASP Top10 \cite{OWASP}. ``Top XX’’ lists have also been generated by security and software vendors who use publicly available metrics and/or proprietary ones \cite{SymnatecReport2019}, \cite{MCAfeeReport2019}. 

% The CWE 
In this work, we undertake a similar exercise (i.e., generate ``Top XX'' list) by providing metrics to calculate the most significant software security weakness types. We do so by considering the CWE, for which we reveal a major bias: the official MDSE equation highly biases frequency and almost ignores severity in generating top lists of varying sizes. As a correction, we apply a double log function to the frequency. We then propose a variety of other improvements, provide top lists of the most significant CWEs for 2019, and provide an analysis of those software security weaknesses.

% Improvement proposals
Previous attempts to improve the CWE include the work by Wu \emph{et. al} \cite{Wu2015CWE} who proposed new definitions of CWEs that are claimed to be substantially more precise and accurate than the current CWE descriptions. Jonathan Spring \emph{et. al} \cite{Jspring2018} suggests reworking the CVSS scoring formula after pointing out some weaknesses in its current form. In \cite{mell2020} the authors propose a suite of additional (to the CWE) metrics for calculating the most signiﬁcant security relevant software flaw types. This is accomplished through creating mashup views combining CWE weakness taxonomies with vulnerability analysis data.


MITRE has also been continually improving the CWE. From its initial status, the project has gone through several iterations to become the CWE in 2006. Follow-on releases over the years refined these software weakness types and their classification trees, while also adding new content such as in 2014 for mobile applications \cite{CWE-history}. In recent years, hardware security issues (with the development of IoT) have become increasingly important concerns, prompting MITRE to add support for hardware weakness in the CWE list \cite{CWE-history}.


% This paper

Our work should be considered as one more step in the continuing improvement process of the CWE. With respect to that, we believe that our contribution is major as it points out a serious bias that is preventing CWE from meeting some of its intended objectives. We propose a fix as well as other improvements.  Our hope is that the community will adopt our newly suggested correction and improvements to the CWE.


==> Archive/AssaneSectionCompressed.tex <==
%%% General security metrics
Modern’s society constant need to improve computer and information security has motivated a widespread interest in deriving metrics for security. Indeed, as stated by Lord Kelvin, \emph{you cannot improve if you cannot measure}. 
%Decision-makers need information about the utility of different security options to make appropriate decisions and to determine how well an organization is meeting its security objectives. Software vendors must provide (to end-users) quantifiable proof that their proposed solutions are achieving the desired security level. End-users must be able to verify such claim. They also need a measuring stick to assess risk related to using a given solution, as risk management requires that one solution be evaluated against an alternate one.
This has led to many efforts devoted to deriving qualitative ways \cite{guide_secu} as well as quantitative ways \cite{ ou2011quantitative} to measure security. The present paper sits within the latter group.

% Critics of security metrics
Providing useful metrics for software security has been identiﬁed as a diﬃcult undertaking mainly because of the lack of a ground truth to assess security metrics. This has prompted members of the software security community to doubt about our ability to succeed in our attempts to quantify security. Bellovin was among the first \cite{Bellovin2006} to argue about the infeasibility of software security metrics. \cite{Cox-limit2008} discusses the limitations of the celebrated ``Risk = Threat × Vulnerability × Consequence'' model that is widely used. In \cite{Verendel2009QuantifiedSI} Verendel presents a critical survey of results and assumptions made in the community to quantify security. 
%After reviewing over 100 articles, he concludes that the validity of most methods is still strikingly unclear. Many reasons explain this invalidity:  lack of validation, lack of comparison against empirical data, and the fact that many assumptions in formal treatments are not empirically well-supported in operational security.

Although we agree that the field of security metrics is a difficult area of scientific research, we believe that acceptable solutions must be found in order to make security decisions and to evaluate whether or not a security posture has improved or declined. The CWE \cite{CWE} is widely agreed to be one of such acceptable solutions. This paper considers the CWE, identifies some of its weaknesses, and proposes  a way to improve it.

%surveys
Despite the doubts raised by some authors,  there has been substantial efforts to produce security metrics. \cite{Verendel2009QuantifiedSI} surveys the literature of security metrics published between 1981 and 2008. More efforts can be found in \cite{Purboyo2011}, \cite{Pendleton2017}, and \cite{MorissonSMS}. 
%This latter survey considers how to measure system-level security by proposing a security metrics framework based on vulnerabilities, defense power, attack or threat severity, and situations (state of system). The authors discuss the state-of-art of existing security metrics and their advantages and disadvantages. They also discuss open research questions in the security metrics research domain and suggest key factors to improve security.

% Discovery tools/methods/DB (Weakness, vulnerability, exploit, attack)
% Prioritizing TOP-X
% Mitigating

Improving software security requires the collaboration of several actors, including: language designers, compiler writers, educators, assurance tool developers, researchers, vulnerability trackers, and software engineers. Such a collaboration cannot succeed if these actors do not ``speak the same language’’. This is what motivated the development and the adoption of widely agreed taxonomies for weaknesses \cite{CWE}, vulnerabilities \cite{CVE}, as well as attacks \cite{CAPEC}. Once broadly accepted definitions and classifications are developed, the key elements pertaining to security can be collected and stored in databases for the needed future analysis. Several such databases have been implemented and are publicly available. They include the  CWE list \cite{NVDCWE}, the CVE list \cite{CVE}, the NVD \cite{NVD}, the exploit DB \cite{ExploitDB}, and the Common Attack Pattern Enumeration and Classification   \cite{CAPEC}. This work is particularly focused on the CWE. It also leverages the CVE and the NVD.

These databases contain sometimes up to thousands of items. From an operational point of view and because of the limited available resources  (manpower, time, money, etc.), one needs to focus on the most ``important’’ items (weakness, vulnerability, exploit, or attack). But finding the most important items requires a metric to compare them.  This has sparked a widespread interest in deriving metrics for security. A number of them can be found in the survey papers \cite{Verendel2009QuantifiedSI}, \cite{Purboyo2011}, \cite{Pendleton2017}, and \cite{MorissonSMS}. The CWE project has also introduced the Common Weaknesses Scoring System (CWSS) \cite{CWSS} and the Common Weakness Risk Analysis Framework (CWRAF) \cite{CWRAF}, which are used in conjunction to provide to an organization with a tailored  list of most important weaknesses. 

Using these metrics, we can generate ``Top XX’’ lists such as the MITRE CWE Top25 \cite{MitreTop25} and the OWASP Top10 \cite{OWASP}. ``Top XX’’ lists have also been generated by security and software vendors who use publicly available metrics and/or proprietary ones \cite{SymnatecReport2019}, \cite{MCAfeeReport2019}. 
In this work, we undertake a similar exercise  by providing top lists of the most significant CWEs for 2019. Furthermore, we provide an analysis of those software security weaknesses.
%metrics to calculate the most significant software security weakness types. 

%We do so by considering the CWE, for which we reveal a major bias: the official MDSE equation highly biases frequency and almost ignores severity in generating top lists of varying sizes. As a correction, we apply a double log function to the frequency. We then propose a variety of other improvements, provide top lists of the most significant CWEs for 2019, and provide an analysis of those software security weaknesses.

% Improvement proposals
Previous attempts to improve the CWE include the work by Wu \emph{et. al} \cite{Wu2015CWE} who proposed new definitions of CWEs that are claimed to be substantially more precise and accurate than the current CWE descriptions. Jonathan Spring \emph{et. al} \cite{Jspring2018} suggests reworking the CVSS scoring formula after pointing out some weaknesses in its current form. In \cite{mell2020} the authors propose a suite of additional (to the CWE) metrics for calculating the most signiﬁcant security relevant software flaw types. This is accomplished through creating mashup views combining CWE weakness taxonomies with vulnerability analysis data.


MITRE has also been continually improving the CWE. From its initial status, the project has gone through several iterations to become the CWE in 2006. Follow-on releases over the years refined these software weakness types and their classification trees, while also adding new content such as in 2014 for mobile applications \cite{CWE-history}. In recent years, hardware security issues (with the development of IoT) have become increasingly important concerns, prompting MITRE to add support for hardware weakness in the CWE list \cite{CWE-history}.


% This paper

Our work should be considered as one more step in the continuing improvement process of the CWE. With respect to that, we believe that our contribution is major as it points out a serious bias that is preventing CWE from meeting some of its intended objectives. We propose a fix as well as other improvements.  Our hope is that the community will adopt our newly suggested correction and improvements to the CWE.


==> Archive/IrenaSection.tex <==
\newcommand{\cwelink}[1]{\href{https://cwe.mitre.org/data/definitions/#1.html}{CWE-#1}}

The mitigated MDSE’ equation represents our metrics for determining the most significant software security weakness types in terms of the CWE. It is intended to combine in an unbiased manner the frequency of a CWE being listed in CVEs  with the severity of these CVEs exploitation. A CWE is one of the most dangerous if it is found frequently consistently in CVEs that are highly severe. A CVE is severe if it is easy to exploit (use the vulnerability in an attack) and with high impact (damage to an affected component).

\subsection{Levels of Abstraction}
The CWE weaknesses model is composed of four layers of abstraction: Pillar, Class, Base, and Variant. There is also the notion of a Compound Element. The abstraction reflects to what extent issues are being described in terms of five dimensions: behavior, property, technology, language, and resource. Variant weaknesses are at the most specific level of abstraction; they describe at least three dimensions. Base weaknesses are more abstract than variants and more specific than classes; they describe two to three dimensions. Class weaknesses are very abstract; they describe one to two dimensions, typically not specific about any language or technology. Pillar weaknesses are the highest level of abstraction. A Compound Element associates two or more interacting or co-occurring CWEs \cite{MitreGlossary}.

\subsection{Ranking Lists}
% What is "It" (first word line 10)?
It contains two pillars (\cwelink{682} and \cwelink{697}) and 36 classes; as well as 81 bases, three variants (\cwelink{415}, \cwelink{416}, and \cwelink{401}), and  two compounds (\cwelink{352} and \cwelink{384}). 
MITRE Top 25 \cite{MitreTop25} ranks CWE items across all the layers of  abstraction from view \cwelink{1003}, where some of  these items have child-parent relationships. It lists seven classes, 16 bases, one variant, and one compound; and there is separate counting for children's occurrences in CVEs and the occurrences of their parent class CWE. For example, the count for the top class \cwelink{119} (rank 1, count 1048) does not include the counts of its children \cwelink{125} (rank 5, count 678) and \cwelink{787} (rank 12, count. 473). Analogously, the count for the class \cwelink{287} (rank 13, count 299) does not include the counts of its children base \cwelink{798} (rank 19, count 91) and base \cwelink{295} (rank 25, count 77). This kind of raking is rather difficult to interpret. Counting and comparing only items that are at the same level of abstraction would be more reasonable.

The NIST Top 20 lists rank view \cwelink{1003} using the mitigated MDSE’ equation while separating pillars and classes from basses, variants, and compounds (Tables  \ref{tab:Top20Classes} \& \ref{tab:Top20Bases}).The Top 20 Classes comprise 19 class CWEs and the pillar \cwelink{682} (rank 9) -- see Table \ref{tab:Top20Classes}. Only three CVEs are directly described with the pillar but it is in the list appears in the list because there is a set of severe CVEs described with its children (see subsection “Next Most Dangerous CWEs”). The Top 20 Bases comprise 17 bases, the variants \cwelink{416} (rank 7) and \cwelink{415} (rank 14), and the compound \cwelink{352} (rank 10) --see Table \ref{tab:Top20Bases}. Each list properly compares items of the same kind, and each CWE from Top 20 Bases is a child of a CWE from Top 20 Classes. However, not all classes follow the same order as their children. One interesting example is \cwelink{74}, which we discuss in section “The Most Dangerous CWEs -- Injection vs Memory Errors”. The only kind of discrepancies left relate the impossibility to inverse the propagation, as it is a surjective function. So, CVEs described by class CWEs do not get reflected in the Top20 Bases list.
\subsection{Ranking Reordered}
There are two main reasons for the reordering of the items in the Top 20 lists (Tables  \ref{tab:Top20Classes} \& \ref{tab:Top20Bases}) compared to the items in Top 25 \cite{MitreTop25}: (1) the Top 25 list is biased towards the frequency of a CWE occurring in CVEs; (2) the Top 20 Classes list counts all basses and classes that are children of the ranked classes.

Top 20 Classes brings in the class CWEs with different weights compared to those in Top 25, as it is generated via the propagation approach from [Peter paper]. \cwelink{89} (SQL Injection) and \cwelink{502} (Deserialization of Untrusted Data) climb up in the Top 20 Basses due to their highest  severities of 8.89 and 9.01. \cwelink{913} (Improper Control of Dynamically-Managed Code Resources) does not even appear in Top 25, as it has only three direct occurrences in CVE. However, it climbs up to first position in Top 20 Classes due to its highest severity of 8.81 and its 188 propagated occurrences. Its main child contributor is base \cwelink{502} with frequency of 83 and severity of 9.01. The Top 25 \cwelink{119} (Improper Restriction of Operations within the Bounds of a Memory Buffer), while widely used with 2745 propagated occurrences in the CVEs, is quite less severe than \cwelink{913} and drops to rank 2 in Top 20 classes. 

All the classes from Top 25 with children from Top 25 appear also in Top 20 Classes: class \cwelink{119} with children base \cwelink{125} and base \cwelink{787}, and class \cwelink{287} with children base \cwelink{798} and base \cwelink{295}. While base \cwelink{120} (a child of \cwelink{119}) comes into Top 20 Bases; the base \cwelink{295} (a child of \cwelink{287}) drops out of Top 20 Bases. Classes that are in Top 25 but do not appear in  Top 20 Classes  are: \cwelink{200} and \cwelink{732}. Basses that are in Top 25 but do not appear in Top 20 bases are \cwelink{79}, \cwelink{476}, \cwelink{772}, \cwelink{426}, \cwelink{295}. 

\subsection{The Two Most Dangerous CWEs: Injection vs Memory Errors}
The two most distinctive groups of weaknesses both in the Top 25 list and the two Top 20 lists are injection and memory errors. However, the use of mitigated MSDE’ and the split in Top 20 Basses (Table \ref{tab:Top20Bases}) and Top 20 Classes (Table \ref{tab:Top20Classes}) considerably reorders them, as well as brings new CWEs and drops some CWEs. 

Injection is the most dangerous type of weakness, represented by \cwelink{89} (SQL Injection), \cwelink{78} (OS Command Injection), \cwelink{94} (Code Injection), and \cwelink{611} (Improper Restriction of XML External Entity Reference), with ranks 1, 4, 6, and 17 respectively (see Table \ref{tab:Top20Bases}). An injection happens when a command string gets assembled partially from input with language-specific special elements and parsed into an invalid construct \cite{bojanova2016bugs}. The invalid constructs for the four most dangerous injection CWEs are respectively SQL Query, OS Command, Code, XML Entity. Top 25 also contains these four CWEs, however the rankings of the first two are 6 and 11 due to the lower frequencies of 397 and 217. The unbiased accounting of their high severity scores of 8.86 and 8.56 moved them several positions up in the Top 20 Bases. In addition, the second ranked in Top 25 \cwelink{79} (Cross-site Scripting), which invalid construct is a generated Web Page, drops out of Top 20 Bases, as although it has the highest frequency of 1571, its severity score of 5.83 is relatively low. The Top 20 Classes brings up also \cwelink{116} (Improper Encoding or Escaping of Output) and CWE 74 (Injection), ranked 14 and 16 (see Table \ref{tab:Top20Classes}). The reason for that is \cwelink{116} is a typical cause of injection and \cwelink{74} is the parent of \cwelink{78}, \cwelink{89}, and \cwelink{94}. Interestingly, the class \cwelink{74} has rank 16 among classes, while its children base \cwelink{89}, \cwelink{78}, and \cwelink{94} are ranked 1, 4, 6 among bases. The frequencies of 2455 for \cwelink{74}, 384 for \cwelink{89}, 194 for \cwelink{78}, and 100 for \cwelink{94}, leave 1777 injection CVEs that are described with CWEs that are either very infrequent or nonsevere. These are \cwelink{79} (Cross-site Scripting) with the low severity of 5.83, \cwelink{88} (Argument Injection) with the low frequency of 6, and \cwelink{91} (XML Injection) with the low frequency of 16. Being not too dangerous they bring the class \cwelink{74} down to rank 16.That same  base \cwelink{79} is ranked 2nd in Top 25 due to the frequency biasing.

The most dangerous memory weaknesses that compete with injection are \cwelink{787} (Out-of-bounds Write) and \cwelink{120} (Classic Buffer Overflow) with ranks 3 and 5 -- see Table \ref{tab:Top20Bases}. Both of them are new to Top 20 Bases compared to Top 25, due to the correction of the frequency bias towards proper reflection of their severity scores of 8.34 and 8.55. Compared to the most dangerous injection weaknesses again while \cwelink{787} is more frequent than \cwelink{89} -- 423 vs 384,-- the severity scores of 8.34 vs 8.89  pushes SQL Injection to the top of the list. The variants \cwelink{416} (Use After Free) and \cwelink{415} (Double Free) with ranks 9 and 14 are peers and main contributing children to \cwelink{672} (Operation on a Resource after Expiration or Release) with rank 4 in Top 20 Classes. They also contribute as grandchildren to class \cwelink{119} through their parent class \cwelink{825} (Expired Pointer Dereference), which is not in view \cwelink{1003}. \cwelink{787}, \cwelink{120}, and \cwelink{125} (Out-of-bounds Read) are the bases contributing to the class \cwelink{119} (Improper Restriction of Operations within the Bounds of a Memory Buffer) with rank 2 in Top 20 Classes. Lastly, class \cwelink{400} (Uncontrolled Resource Consumption) with rank 15 is mostly directly assigned to CVEs (see Table \ref{tab:Top20Bases}).

The majority of the base CWEs in this group  are memory use weakness -- \cwelink{120}, \cwelink{125}, and \cwelink{787} are buffer overflow (out of bounds read or write); \cwelink{416} is use after free (use of deallocate memory through a dangling pointer). Another base CWE is a memory deallocation weakness: \cwelink{415} is double free (deallocate of already deallocated memory). Class \cwelink{119} is a general memory corruption weakness, which includes buffer overflow, use after free and double free. Yet, another class CWE from this group is a memory allocation weakness: \cwelink{400} is memory overflow (stack/heap  exhaustion) \cite{BFMem}. 

Compared to Top 25, the mitigated MDSE’ brings up several injection weaknesses with much higher severity than that of any memory weaknesses. The related CVEs analysis confirms that the injection CVE are easier to exploit and with higher impact. An injection directly leads to arbitrary command, code, or script execution.Once a SQL injection is in place, there is no need of additional sophisticated attack crafting or use of glitches in the system. While It takes considerable extra effort for an attacker to turn a buffer overflow into an arbitrary code execution. The attacker also needs exceptional skills in applying spraying memory techniques.and more [SoK: War on Memory paper]. The possible damage from a SQL injection is also very high. It may expose huge amounts of structured data, which is always more valuable than raw data. Well formed structured data is easy to read, sort, search, and make sense of it. An attacker could modify a database -- insert, update, delete data, execute admin operations, recover file content, and even issue OS commands to the operating system \cite{OWASPInjection}.

\subsection{Next Most Dangerous CWEs}
Next groups of weaknesses in Top 20 Bases and Classes relate to file input and upload, authentication,  randomization, cryptography, arithmetics and conversion, and input validation. 
The most dangerous file input and upload weaknesses are base \cwelink{502} (Deserialization of Untrusted Data) and base \cwelink{434} (Unrestricted Upload of File with Dangerous Type) with ranks 2 and 8, respectively. They are the main contributors to class \cwelink{913} and class \cwelink{669} with ranks 1 and 3, respectively.

Top 20 Classes brings up also the randomization weaknesses class \cwelink{330} (Use of Insufficiently Random Values) with rank 5, which is mostly directly assigned to CVEs. 
The most dangerous authentication weakness is base \cwelink{798} (Use of Hard-coded Credentials) with rank 7; which is one of the contributors to the class \cwelink{287} (Improper Authentication) with the same rank 7 in Top 20 Classes.

The most dangerous cryptography weakness is base \cwelink{352} (Cross-Site Request Forgery -- CSRF)with rank 10, which relates to bugs in data verification. Top 20 Classes list also class \cwelink{326} (Inadequate Encryption Strength) with rank 18, which is directly assigned to 35 CVEs with severity 7.24.

The most dangerous arithmetics and conversion weaknesses are \cwelink{190} (Integer Overflow or Wraparound) and \cwelink{191} (Integer Underflow) with rank13 and 20, which are the main contributors to the pillar \cwelink{682} (Incorrect Calculation) with rank 9 in Top 20 Classes. Note that only three CVEs are directly described with the pillar \cwelink{682}, but it is in the Top 20 Classes list due to the set of severe CVEs described with its children bases \cwelink{131} (Incorrect Calculation of Buffer Size), \cwelink{190} (Integer Overflow or Wraparound), and \cwelink{191} (Integer Underflow -- Wrap or Wraparound) with severities 9.8, 7.95, and 8.47, respectively. \cwelink{131} though does not appear in the Top 20 Basses, as it has only one occurrence in the CVEs.
The most dangerous input validation weakness is \cwelink{129} (Improper Validation of Array Index) with rank 16.

\subsection{Dependent on CWE, CVE, and NVD}
Both Top 25 and Top 20 rankings heavily depend on how NVD assigns CWEs to particular CVEs. The CWE selection is restricted to view \cwelink{1003}. The lack of enough information about a CVE or the lack of a more specific CWE may lead to the CVE described with the closest class CWE or even with a pillar CWE. For example, It makes sense for class \cwelink{119} to be used for the memory corruption CVE-2019-7098, as there is not much  information, no code, no details about it -- it could be any memory use error or a double free. .However, there is enough information about  the use after free CVE-2019-15554 and it still gets described  with class \cwelink{119}, as there is no appropriate base CWE. A close base CWE is \cwelink{416} (Use After Free), but it does not really reflect memory safe languages like Rust. It is also possible for a class CWE to be assigned to a CVE even when a specific  base CWE is available. For example, the stack buffer overflow write CVE-2019-14363 is assigned class \cwelink{119}, although there is plenty of information and appropriate bases \cwelink{121} and \cwelink{120}. 

